Babylon: Reusing Bitcoin Mining to Enhance Proof-of-Stake Security

Bitcoin is the most secure blockchain in the world, supported by the immense hash power of its Proof-of-Work miners, but consumes huge amount of energy. Proof-of-Stake chains are energy-efficient, have fast finality and accountability, but face several fundamental security issues: susceptibility to non-slashable long-range safety attacks, non-slashable transaction censorship and stalling attacks and difficulty to bootstrap new PoS chains from low token valuation. We propose Babylon, a blockchain platform which combines the best of both worlds by reusing the immense Bitcoin hash power to enhance the security of PoS chains. Babylon provides a data-available timestamping service, securing PoS chains by allowing them to timestamp data-available block checkpoints, fraud proofs and censored transactions on Babylon. Babylon miners merge mine with Bitcoin and thus the platform has zero additional energy cost. The security of a Babylon-enhanced PoS protocol is formalized by a cryptoeconomic security theorem which shows slashable safety and liveness guarantees.

==> 5_security-features.tex <==
\subsection{Security Features}
\label{sec:security-features}

In brief, the security features of \chain are:
\begin{enumerate}
    \item \chain allows each  PoS chain's client to specify its desired Bitcoin security {\em in addition to} the native security of the PoS chain, by waiting for the timestamp of its transaction to be sufficiently deep in the \chain chain, signifying a significant passage of time (Figure \ref{fig:attack-eg}(a)). This finalization rule is analogous to the $k$-deep confirmation rule in Bitcoin. It is particularly useful in the bootstrapping phase of a PoS chain when the native security is weak. Just like in Bitcoin, the finalization rule can be specified on a transaction-by-transaction basis; a transaction that does not need the additional Bitcoin security can still enjoy the native fast finalization feature of the PoS chain. 
    \item \chain protects the PoS chains against long range attacks. A long range attack is mounted by building a long fork using old coins, but such a long fork will have much newer timestamps on Babylon compared to the canonical chain and will be rejected by the validators (Figure \ref{fig:attack-eg}(c)). Thus, \chain removes the need to recourse to social consensus as in Ethereum 2.0 and other PoS chains, and this is particularly useful for smaller blockchains which do not yet have a strong community to achieve social consensus. Moreover, the stake lockup period can be dramatically reduced. 
    \item \chain protects against transaction censorship and protocol stalling in PoS chains by allowing a censored transaction to be timestamped on the \chain chain. Once the timestamp becomes sufficiently deep in the Babylon chain, signifying a significant passage of time, validators will have to vote for that transaction otherwise they will be slashed.
    
\end{enumerate}

A more precise statement of the security of \chain is given in Section \ref{sec:sec-analysis} in terms of a security theorem. 

In addition to these basic security features, \chain can also provide other features by virtue of the fact that it is  a platform used by multiple PoS chains. For example. \chain can  provide global fair ordering across the PoS blockchains it supports to facilitate cross-chain communication.

